Lumen: A Machine Learning Framework to Expose Influence Cues in Text

Phishing and disinformation are popular social engineering attacks with attackers invariably applying influence cues in texts to make them more appealing to users. We introduce Lumen, a learning-based framework that exposes influence cues in text: (i) persuasion, (ii) framing, (iii) emotion, (iv) objectivity/subjectivity, (v) guilt/blame, and (vi) use of emphasis. Lumen was trained with a newly developed dataset of 3K texts comprised of disinformation, phishing, hyperpartisan news, and mainstream news. Evaluation of Lumen in comparison to other learning models showed that Lumen and LSTM presented the best F1-micro score, but Lumen yielded better interpretability. Our results highlight the promise of ML to expose influence cues in text, towards the goal of application in automatic labeling tools to improve the accuracy of human-based detection and reduce the likelihood of users falling for deceptive online content.

==> sections/old_3-design_impl.tex <==
\section{Lumen Design and Implementation}
\label{sec:design-impl}

\needsupdate
This section describes the design and implementation of Lumen,  our proposed two-level learning-based framework to expose the following influence cues in phishing emails: (i) persuasion, (ii) framing (gain/loss), and (iii) emotional salience. 
Persuasion refers to a set of principles that influence how people concede or comply with requests. Cialdini~\cite{Cialdini1993,Cialdini2001Science} has identified six of these principles, which are used in Marketing: authority, scarcity, reciprocation, social proof, liking, and consistency. For example, people tend to comply with requests or accept arguments made by figures of authority. Framing refers to the presentation of a message (e.g., health message, financial options, and advertisement)  as implying a possible gain (i.e.,  possible benefits of performing the action) vs. implying a possible loss (i.e., costs of not performing a behavior)~\cite{Rothman1997-jx,Kuhberger1998-cs,Kahneman1979-jz}. Framing can affect decision-making and behavior. Work by Kahneman and Tversky \cite{ Kahneman1979-jz } on loss aversion supports the human tendency to prefer avoiding losses over acquiring equivalent gains. This tendency implies that framing a message as a loss may be more impactful than framing it as a gain. Emotional salience refers to both valence (positive to negative) and arousal (arousing to calming) of an experience or stimulus~\cite{Russell1980-og,Peace2012-dm,Kircanski2018-rh}. Deception detection is reduced for emotional compared to neutral stimuli~\cite{ Peace2012-dm }. Similarly, persuasion messages that generate high compared to low arousal lead to poorer consumer decision-making~\cite{ Kircanski2018-rh}. Emotional salience may impair full processing of deceptive content and high arousal content may trigger \emph{System 1}, the fast, shortcut-based brain processing mode \cite{Ariely2009-op}. 


Exposing presence of persuasion and framing is tackled  as a multi-labeling document classification problem, where zero, one, or more labels can be assigned to each document. 
%For example, a phishing email can employ more zero, one or more principles of persuasion and framing and Lumen’s goal is to expose their presence using machine learning methods. 
Due to recent developments in natural language processing, emotional salience is an input feature that Lumen exposes leveraging sentiment analysis.  Note that  Lumen's goal is not to distinguish phishing vs. benign email, but to expose different principle of influence applied  in the phishing email.

Figure \ref{fig:lumen} illustrates Lumen’s two-level hierarchical learning- based architecture. On the first level, the following predictive features are generated from the raw phishing text: (i) topical structure inferred by topic modeling, (ii) LIWC features related to influence keywords~\cite{pennebaker2015development}, and (iii) emotional salience features learned via sentiment analysis ~\cite{Hutto2014}. On the second level, a general-purpose ML algorithm is used to predict the principle(s) of persuasion and  framing applied to the message.

\begin{figure*}[h]
	\centering
	\includegraphics[width=\textwidth]{fig/lumen.JPG}
	\caption{\needsupdate Lumen's two-level architecture. Pre-processed email text undergoes sentiment analysis for extraction of emotional salience, LIWC analysis for extraction of features related to influence keywords, and topic modelling for structural features. These features are inputs to ML analysis for prediction of principle(s) of persuasion  and the framing applied to the message.}
	\label{fig:lumen}
\end{figure*}

\textbf{Topic structure features.}
Probabilistic topic modeling algorithms are often used to infer the topic structure of unstructured text data~\cite{Steyvers2007,BleiBook2009}, which in our case  are  phishing emails.
Generally, these algorithms assume that a collection of documents, also named as corpus, are created following the generative process.
Suppose that there are $D$ documents in the corpus $\mathcal{C}$ and each document $d=1,...,D$ has length $m_d$.
Also suppose that there are in total $K$ different topics in the corpus and the vocabulary $\mathcal{V}$ includes $V$ unique words.
The relations between documents and topics are determined by conditional probabilities $P(t|d)$, which specify the probability of topic $t=1,...,K$ given document $d$.
The linkage between topics and unique words are established by conditional probabilities $P(w|t)$, which indicate the probability of word $w=1,...,V$ given topic $t$.
According to the generative process, for each token $w(i_d)$, which denotes the $i_d$-th word in document $d$, we will first obtain the topic of this token, $z(i_d)=t$, according to $P(t|d)$. 
With the obtained $z(i_d)$, we then draw the a word $w(i_d)=w$ according to $P(w|t=z(i_d))$ .

In this work, we leveraged Latent Dririchlet Allocation (LDA), one of the most widely used topic modeling algorithms, to infer topic structure in phishing emails~\cite{Blei2003lda}.
In LDA, both $P(w|t)$ and $P(t|d)$ are assumed to have Dirichlet prior distributions. 
Given the phishing email dataset, which is the evidence to the probabilistic model, the goal of LDA is to infer the most likely conditional distribution $\hat P(w|t)$ and $\hat P(t|d)$, which is usually done by either variational Bayesian approach~\cite{Blei2003lda} or Gibbs Sampling~\cite{Griffiths2004}. 
In Lumen, the conditional probabilities $\hat P(t|d)$ represent the topic structure of the phishing email dataset.

\textbf{LIWC Influence Features.} Human beings use language to convey their thoughts, intentions, and emotions, with words serving as basic building blocks of languages. Thus, the way different words are used in unstructured text data  provide meaningful information to streamline our understanding of the use of influence cues in text data. 

Lumen leverages LIWC, a natural language processing framework that connects commonly-used words with categories~\cite{tausczik2010psychological, pennebaker2015development},  to retrieve influence features of phishing emails to aid  ML classification. LIWC includes more than 70 different categories in total, such as Perceptual Processes, Grammar, and Affect, and more than 6,000  common words. However, not all the categories are related to  influence. After careful inspection, we manually selected seven  categories as features related to influence for Lumen. 
For persuasion we selected the category ``time'' (related to scarcity). 
For emotion, we selected the categories ``anxiety,'' ``anger,'' and ``sad.'' For framing, we selected the categories ``reward'' and ''money'' (gain) and ``risk'' (loss).
Table \ref{tab:liwc_cats} shows word examples for each chosen LIWC category and the number of words in each category.

\begin{table}[h]
	\caption{\needsupdate? LIWC categories and keywords.}
	\begin{tabular}{c|c|c}
		\hline
		LIWC category & Keywords             &  Total number of words     \\ \hline
		anxiety           & afraid, anxious           &  92               \\ \hline
		anger         & abuse, aggress            &  176              \\ \hline
		sad           & abandon, alone            &  98               \\ \hline
		
		time          & after, afternoon          &  251              \\ \hline
		reward        & access, achieve           &  75               \\ \hline
		risk          & alarm, abstain            &  81               \\ \hline
		money         & account, auction          &  167              \\ \hline
	\end{tabular}
	\label{tab:liwc_cats}
\end{table}

We denote the collection of all six chosen  LIWC  categories as set $\mathcal{S}$.
Given a phishing email document $d$ with document length $m_d$ from the phishing email corpus $\mathcal{C}$, to build the LIWC  feature $X^{LIWC}_{i,d}, \forall  i \in \mathcal{S}$,  we first count the number of words in email $d$ belonging to the LIWC  category $i$, denote as $n_{i,d}$, then normalize the raw word count with the document length:
\begin{equation}
X^{LIWC}_{i,d}=\frac{n_{i,d}}{m_d}, \forall  i \in \mathcal{S}, d \in \mathcal{C}.
\end{equation}

\textbf{Emotional Salience by Sentiment Analysis.}
%Emotional salience refers to both valence (positive to negative) and arousal (arousing to calming) of an experience or stimulus~\cite{russell1980circumplex}. 
Deception detection is reduced for emotional compared to neutral stimuli~\cite{peace2012}. 
%Similarly, persuasion messages that generate high compared to low arousal lead to poorer consumer decision-making~\cite{Kircanski2018}. 
%Emotional salience may impair full processing of deceptive content and high arousal content may trigger System 1, the fast, shortcut-based brain processing mode~\cite{ariely2009large}, potentially leading to poor deception detection.
In this work we used a pre-trained rule-based model, VADER, to extract the emotional salience from a phishing email~\cite{Hutto2014}.
Given a phishing email document $d$, VADER provides the level of positive emotion, $E^{pos}_d$, and the level of negative emotion, $E^{neg}_d$.
Both levels of emotion range from 0 to 1, where a small value means low emotional levels and a large number means high emotional levels. Therefore, emotional salience is both an input feature to the learning model and one of Lumen’s outputs (see Figure \ref{fig:lumen}). 

\textbf{Machine Learning to Predict Persuasion and Framing.} Lumen's second level corresponds to the application of a general-purpose ML algorithm for document classification. %For the analysis done in this paper, we choose Random Forest (RF) to use the features generated during the first level analysis to predict the existence of principles of influence given a phishing email: framing and persuasion. 
Even though Lumen is general enough to allow application of any general purpose algorithm, in this presentation, we applied Random Forest (RF) because it can provide the level of importance for each input predicative feature without additional computational cost, which aids in model understanding. For instance, with RF we can discover which topic or LIWC feature are the most important. Another advantage of RF is its robustness to the magnitudes of input predicative features, i.e., RF does not need feature normalization. %One opposite example is Support Vector Machine, which requires all features to have approximately the same level of magnitude to perform well. 
%Please note that emotional salience is a feature that can be extracted from the text and, therefore, does not need to be predicted. 
The input features for the ML algorithm are summarized in Table~\ref{table_input_feature}.

Assume the collection of all  principles of influence is $\mathcal{P}$, the output/target of the ML algorithm is the binary indicators $I_{p,d}, \forall p \in \mathcal{P}$ to show if principle $p$ appears in phishing email $d$.
%We use the grid search approach to fine-tune the parameters in the RF model and follow the cross-validation to overcome the over-fitting issue of the model (more details can be found in Section~\ref{results}).

\begin{table}[h]
	\caption{Input features for phishing email $d$.}
	\begin{tabular}{c|c|c}
		\hline
		Features &                Symbols   & Number of features       \\ \hline
		Topic           & $P(t|d), i=1,...,K$           &  $K$               \\ \hline
		LIWC          &       $X^{LIWC}_{i,d}, \forall i \in \mathcal{S}$      &  7              \\ \hline
		Emotion            &     $E^{pos}_d$, $E^{neg}_d$        &  2              \\ \hline
	\end{tabular}
	\label{table_input_feature}
\end{table}

==> sections/old_4-evaluation.tex <==
% ********************************************
\section{Evaluation}
\label{sec:eval}
% ********************************************
\ToDo{Split this section into Methodology and Results}

This section details Lumen’s evaluation. We first describe the methodology used to generate the labeled dataset of 
\changed{disinformation, hyperpartisan media, and center-leaning media} 
in our analysis; then, we provide a quantitative analysis of the dataset. Next, we describe our evaluation metrics, how we pre-processed the dataset for Lumen analysis, training/testing procedures, and the results of Lumen classification in comparison to other ML algorithms.


% ********************************************
\subsection{\changed{Curating the Dataset}}
% \subsection{The Labeled Dataset}
% ********************************************
\changed{We composed a diverse dataset in terms of influence cues and persuasion tactics by gathering different types of information from multiple sources that we split into three groups: $1,082$ pieces of text containing disinformation and/or deception tactics (Group A), $1,003$ hyperpartisan media news from politically right- and left-leaning publications (Group B), and $974$ center mainstream media news (Group C). Our dataset therefore contained $3,059$ pieces of text in total.}

\changed{For Group A (disinformation/deception pieces), we mixed $492$ Facebook ads created by the Russian Internet Research Agency (IRA), $130$ fake news, and $460$ phishing emails, as follows.}

\noindent
\changed{\textbf{Facebook IRA ads}. 
We leveraged a dataset of 3,517 Facebook ads created by the Russian IRA and made publicly available to the U.S. House of Representatives Permanent Select Committee on Intelligence~\cite{noauthor_undated-wp} by Facebook after internal audits. These ads were a small representative sample of over 80K organic content identified by the Committee and are estimated to have been exposed to over 126M Americans between June 2015 and August 2017. After discarding ads that did not have text entry, the dataset was decreased to 3,286 ads, which were mostly (52.8\%) posted in 2016 (U.S. election year), followed by 29.2\% in 2017, and the remaining 18.0\% in 2015. We randomly selected $492$ of these ads to be included as part of Group A.}

\noindent
\changed{\textbf{Fake news}. 
We leverage a publicly available~\footnote{\url{https://ieee-dataport.org/open-access/fnid-fake-news-inference-dataset#files}} dataset of nearly 17K news labeled as \emph{fake} or \emph{real} collected by Sadeghi et al.~\cite{fbzd-sw81-20} from \url{PoliticFact.com}, a reputable source of fact-finding in which a news team and fact-finding experts evaluate political news articles published in various sources (e.g., CNN, BBC, Facebook). We randomly selected $130$ \emph{fake} news ranging from $110-200$ words to be included as part of Group A. These items were dated from 2007 to 2020.}

\noindent
\changed{\textbf{Phishing emails}.}
To gather our  dataset, we collected approximately  15,000 known phishing emails  from multiple public sources~\cite{Smiles2019Phishing, Pittsburgh2019Alerts, Minnesota2019Phishing, UCLA2019Phish, Penn2019Phish, Lehigh2019Recent, UA2019Phishing, Michigan2019Phish}. Individual web-crawlers were written to gather these phishing emails from each of the websites and store them as HTML text documents for analysis. The web-parsed emails were then cleaned and formatted to remove errors, noise (e.g., images, HTML elements), and any extraneous formatting so that only the raw email text remained. Only text indentations and paragraph formatting were retained. \changed{We randomly selected $460$ of these emails ranging from $50-150$ words to be included as part of Group A.}

\changed{
For Groups B (hyperpartisan media news) and C (center mainstream media news), we used a public dataset~\footnote{\url{https://components.one/datasets/all-the-news-2-news-articles-dataset/}} comprised of 2.7M news articles and essays from 27 American publications dated from 2013 to early 2020. We first selected articles ranging from $50-200$ words and then classified them as \emph{left}, \emph{right}, or \emph{center} news according to the AllSides Bias Rating~\footnote{\url{https://www.allsides.com/media-bias/media-bias-ratings}}. 
For inclusion in Group B, we randomly selected $506$ \emph{right} news and $497$ \emph{left} news; the former were dated from 2016 to 2017 and came from two publications (Breitbart and National Review) while the latter were dated from 2016 to 2019 and came from six publications (Buzzfeed News, Mashable, New Yorker, People, VICE, and Vox). To compose Group C, we randomly selected $974$ \emph{center} news from all seven publications (Business Insider, CNBC, NPR, Reuters, TechCrunch, The Hill, and Wired) dated from 2014 to 2019.
}


% ********************************************
\subsubsection{\changed{Coding Process}}
% ********************************************
\changed{
We then developed coding categories and a codebook based on Cialdiani’s principles of influence~\cite{cialdini1993psychology}, subjectivity/objectivity, and gain/loss frames~\cite{kahneman1980prospect}. These categories have been previously used in \XXX \ToDo{Insert our prior phishing works here}, and were adapted for the purposes of this study. Next, we held an initial training session with nine undergraduate students. The training involved a thorough description of the coding categories, their definitions and operationalizations, as well as a workshop-style training where coders labeled a small sample of the texts to get acquainted with the coding platform, the codebook, and the texts. Coders were instructed to read the text at least twice before starting the coding to ensure they understood it. After that, coders were asked to share their experiences labeling the texts and to discuss any issues or ask any questions about the process. After this training session, two intercoder reliability pretests were conducted; in the first pretest, coders independently co-coded a sample of $20$ texts, and in the second pretest, coders independently co-coded a sample of $40$ texts. After each one of these pretests, a discussion and new training session followed to clarify any issues with the categories and codebook.
}

\changed{
Following these additional discussion and training sessions, coders were then instructed to co-code $260$ texts which served as our intercoder reliability sample. To calculate intercoder reliability, we used three indexes. \emph{Cohen’s Kappa} and \emph{Percent of Agreement} ranged from $0.40$ to $0.90$ and 66\% to 99\%, respectively, which was considered moderately satisfactory. Due to the nature of the coding and type of texts, we also opted to use \emph{Perrault and Leigh’s index} because (a) it has been used in similar studies that also use nominal data~\cite{fuller2014lights, hove2013newspaper, morey2016measures, rice2018frequent}; (b) it is the most appropriate reliability measure for $0/1$ coding (i.e., when coders mark for absence or presence of given categories), as traditional approaches do not take into consideration two zeros as agreement and thus penalize reliability even if coders disagree only a few times~\cite{perreault1989reliability}; and (c) indexes such as Cohen’s kappa and Scott’s pi have been criticized for being overly conservative and difficult to compare to other indexes of reliability~\cite{lombard2002content}. Perrault and Leigh’s index ($I_r$) returned a range of $0.67$ to $0.99$, which was considered satisfactory. Finally, the remaining texts were divided equally between all coders, who coded all the texts independently using an electronic coding sheet in Qualtrics.
}

% ********************************************
\subsubsection{\changed{Coding Categories}}
% ********************************************
\changed{
The coding categories were divided into three main concepts: \emph{principles of influence}, \emph{objectivity/subjectivity}, and \emph{gain/loss framing}. For all categories in the study, coders marked for the absence ($0$) or presence ($1$) of the category. The principles of influence were based on~\cite{cialdini1993psychology} work and consist of the following six principles: i) authority or expertise, ii) reciprocation, iii) commitment and consistency, iv) liking, v) scarcity, and vi) social proof. The authors added subcategories to the principles of commitment (i.e., indignation and call to action) and social proof (i.e., admonition) because an initial perusal of texts revealed consistent usage across texts. \emph{Subjectivity} refers to sentences that contain personal opinion, emotion, or judgment, while \emph{objectivity} refers to sentences with factual information, based on evidence, or when evidence is presented. \emph{Gain and loss framing}~\cite{kahneman1980prospect} refer to the presentation of a message (e.g., health, financial options, advertisement, etc.) as implying a possible gain (i.e., refers to possible benefits of performing a behavior) vs. implying a possible loss (i.e., refers to the costs of not performing a behavior). Finally, coders also coded for the presence or absence of \emph{attribution of guilt}, which occurs when the text references an ``another'' (who/what) for the wrong/bad things happening, and the use of \emph{emphasis}, which refers to the use of all caps text, exclamation points (either one or multiple), several question marks, bold text, italics text, or anything that is used to call attention in text. 
}

% ********************************************
\subsection{Quantitative Analysis}
% ********************************************
\needsupdate
Since persuasion and framing are orthogonal directions in the influence space, we considered them separately in this analysis. Note that our coders have not found, based on the coding manual, any phishing email leveraging the principle of reciprocation, which may be due to the limited size of our dataset or may be a reflection of the phenomenon itself. 
Reciprocation might be a principle that does not lend itself well to be applied in text, as it requires giving something to the recipient first and expecting a reciprocation action later.

We found that 4\% of the emails in the dataset did not use any principle of persuasion and that 5\% of the emails use three or more principles of persuasion (Figure~\ref{fig_stats_persuation}-a). More than half of the phishing emails apply only one principle of persuasion, and 37\% of the emails leverage two principles. We hypothesize that these findings may reflect the potential appeal or popularity of phishing emails of moderate complexity. Phishing emails constructed without any principle of persuasion are too simple to convince the receiver, while emails with multiple principles of persuasion might end up being long, which are more time-consuming to write (for attackers) and to read (for receivers). Further, considering only persuasion, Figure~\ref{fig_stats_persuation}-b shows that authority and scarcity were the most prevalent principles appearing, respectively, in 81\% and 50\% of the emails.

\begin{figure}[h]
	\centering
	\includegraphics[width=.75\columnwidth,trim={0 0 0 0.2cm}, clip]{fig/multilabel_emails/fig02_persuation_hist_singleInAll}
	\caption{\needsupdate Principles of persuasion in the phishing dataset.}
	\label{fig_stats_persuation}
\end{figure}

The majority of phishing emails (74\%) was framed exclusively as either gain or loss, 23\% of phishing emails do not include any framing at all, and only 1\% of the emails used both gain and loss framing in the same message. We also found that loss was much more prevalent than gain: about half of all phishing emails (48\%) applied loss, while only 28\% invoke in the user the possibility of a gain.
% \begin{figure}[h]
% 	\centering
% 	\includegraphics[width=.6\columnwidth]{fig/multilabel_emails/fig01_framing_hist_singleInAll}
% 	\caption{Framing (Gain/Loss) in the phishing dataset.}
% 	\label{fig_stats_framing}
% \end{figure}
When considering all principles of influence in Fig.~\ref{fig_influence_count_per_email}, which combines persuasion and framing, most of  emails used two (in 43\% of all phishing emails) or three (32\%) influence principles. Only 20\% of all emails leveraged a single influence principle, which was significantly less compared to Fig.~\ref{fig_stats_persuation}-a. %and \ref{fig_stats_framing}-a, 
% where principles of persuasion are considered separately.


\begin{figure}[h]
	\centering
	\includegraphics[width=.75\columnwidth,trim={0 0 0 0.2cm}, clip]{fig/multilabel_emails/s03_a_influence_count_per_email}
	\caption{\needsupdate Histogram of principles of influence in the phishing dataset.}
	\label{fig_influence_count_per_email}
\end{figure}

%Moreover, Figure~\ref{app_fig_top_single_influence_in_all}, which combines 
Figure~\ref{fig_stats_persuation}-b % and ~\ref{fig_stats_framing}-b 
shows that authority was the most popular principle of influence, followed by scarcity. %y, loss, and gain. And 
These top principles of influence were used much more frequently than the remaining three principles of influence (liking, commitment, and social proof), which gives evidence of the highly imbalanced application of principles of influence in  real phishing campaigns.

%\begin{figure}[h!]
%	\centering
%	\includegraphics[width=.9\columnwidth]{fig/multilabel_emails/s03_b_top_single_influence_in_all}
%	\caption{Popularity of principles of influence in phishing dataset}
%	\label{app_fig_top_single_influence_in_all}
%\end{figure}

Next, we investigated  how persuasion and framing were used in phishing emails applying one, two, and three principles of influence respectively. We divided all phishing emails according to the number of principles of influence in their text---that is, phishing emails with different complexity levels (see Figure~\ref{fig_influence_count_per_email}). 
Here, we only investigated email categories covering more than 10\% of all emails. 
We first focused on  simple emails that  used only one influence of principle, as shown in Figure~\ref{fig_single_influence_in_single}.
Authority  was the most popular, with 60\% prevalence.
%, which corroborates data shown in Figure~\ref{app_fig_top_single_influence_in_all} where authority  was also the most popular principle.
However, there is evident change in the usage of  gain and loss.
%when we compare Figures~\ref{fig_single_influence_in_single} and ~\ref{app_fig_top_single_influence_in_all}. 
For all emails,  loss  was used much more often than the gain  (48\% $>$ 28\%), %in Fig.~\ref{fig_stats_framing}-b), 
while within the emails using single influence principle, gain  was ten times more popular than loss  (20\% $>$ 2\%). %in Fig.~\ref{fig_single_influence_in_single}).
The difference suggests that in  simple phishing emails (using only one principle of influence) attackers might be attempting to lure users to potential financial gain when users act on the email.


\begin{figure}[h!]
	\centering
	\includegraphics[width=.75\columnwidth]{fig/multilabel_emails/s05_a_top_single_influence_in_single}
	\caption{\needsupdate Prevalence of principles of influence---emails applying one principle.}
	\label{fig_single_influence_in_single}
\end{figure}






\begin{figure}[h!]
	\centering
	\includegraphics[width=.75\columnwidth,trim={0 0 0 0.2cm}, clip]{fig/multilabel_emails/s06_c_top_influence_pair_in_pair}
	\caption{\needsupdate Prevalence of principles of influence---emails applying two principles.}
	\label{fig_influence_pair_in_pair}
\end{figure}




In Figure~\ref{fig_influence_pair_in_pair}, we consider emails with moderate level of complexity, using a pair of principles of influence.
Note that Figure~\ref{fig_influence_pair_in_pair} only shows the top five influence pairs, which covers more than 93\% of all the moderately complex emails using influence principle pairs (the total number of influence pairs is 42). The authority-loss  pair was the most popular, covering 54\% of emails with influence principle pair. Also,  loss was far more popular than  gain, which disagrees with emails with single influence principle in Figure~\ref{fig_single_influence_in_single}.
This gives evidence that for relatively complex emails, attackers might prefer to combine a request from an authoritative figure implying a potential loss to the user if users do not  perform a desired action, such as clicking a link.


\begin{figure}[h!]
	\centering
	\includegraphics[width=.75\columnwidth]{fig/multilabel_emails/s07_d_top_influence_triplet_in_triplet}
	\caption{\needsupdate Prevalence of principles of influence---emails applying three principles.}
	\label{fig_influence_triplet_in_triplet}
\end{figure}


The usage of principles of influence  for emails applying three principles is shown in Figure~\ref{fig_influence_triplet_in_triplet}.
The authority-loss-scarcity triplet was the most popular.
In this case,  loss  was much more prevalent than the gain, corroborating what we found for their usage  in Figure ~\ref{fig_influence_pair_in_pair}.


In sum, authority, scarcity, loss, and gain  are the top four principles among all phishing emails (each principle covering more than 20\% of emails).
%, as shown in Fig.~\ref{app_fig_top_single_influence_in_all}.
However, the use of each of the top principles varies across emails with different levels of complexity. Authority was the most popular principle among all types of emails. When the level of complexity of phishing emails grows, the popularity of gain dropped, but that of scarcity and loss increased dramatically.

\subsection{Evaluation Metrics}
\needsupdate
We used the $F1$-score (a function of precision and recall) to evaluate Lumen's performance, following the work by Ramage et al. \cite{Ramage2009} and van der Heijden et al.~\cite{VanderHeijden2019}. 
% Mathematically, precision is defined as 
% \begin{equation}
% 	P=\frac{TP}{TP+FP},
% \end{equation}
% where $P$ denotes precision, $TP$ is the true positive and $FP$ is the false positive.
% In the case of single-labeling document classification, true positive represents the number of selected objects that are relevant and false positive means the number of selected objects that are irrelevant. 
% Thus, $TP+FP$ is the total number of objects being selected. 
% On the other hand, recall is expressed as
% \begin{equation}
% 	R=\frac{TP}{TP+FN},
% \end{equation}
% where $R$ is recall and $FN$ denotes false negative 
%For single-labeling document classification, false negative 
% (the number of unselected objects that are actually relevant; consequently, $TP+FN$ is the total number of relevant objects).
% However, neither precision or recall alone can provide a full picture of the performance of a classification algorithm.
% Here we consider two extreme cases. In the first example, one classification algorithm is very conservative and only selects one single object with the highest likelihood of being relevant. This conservative algorithm is likely to achieve a high precision score but a poor recall score. In the second example, one classification algorithm is very progressive and will select all objects as relevant. This progressive algorithm is likely to achieve a poor precision score, but full recall score. 
% Therefore, we need to find a balance between precision and recall, and the $F1$-score provides such a tradeoff,  being defined as:
In order to find a balance between precision and recall, the $F1$-score provides is used and defined as:

\begin{equation}
	F=\frac{2PR}{P+R},
\end{equation}
where $F$ denotes $F1$-score, $P$ is precision and $R$ represents recall.
We should note that the comparison of $F$ scores is only meaningful under the same experiment setup. 
It will be uninformative to compare F scores from distinctive experiments in different pieces of work in the literature due to varying experiment conditions. $F1$-score can be easily calculated for single-labeling classification problems, where each document will only be assigned to one label. 
However, in our work, we are dealing with a multi-labeling classification problem, which means that no limit is imposed on how many labels each document can include.
Thus, we employed two variations of the $F1$-score to quantify the overall performance of the learning algorithm, i.e., the macro $F1$-score and the micro $F1$-score.
The macro average of $F1$-score  computes the $F1$-score for each category, and obtains their unweighted value for each category.
The macro $F1$-score does not take data imbalance into consideration. The micro average of $F1$-score calculates the $F1$-score globally by counting the total $TP$ (selected objects that are relevant), total $FN$ (unselected objects that are relevant) and total false positives (selected objects that are irrelevant) for all classes.

\subsection{LIWC Features of Influence}
\needsupdate
In this section, we explore whether LIWC features (related to influence) have indicative powers to predict the principles of influence using Figs.~\ref{app_fig_feature_vs_weapon_anx_liwc}--\ref{app_fig_feature_vs_weapon_risk_liwc}.
%, we plot each features against influence  principles in Appendix.~\ref{sec_appendix}.
Figure~\ref{app_fig_feature_vs_weapon_anx_liwc} shows that loss has a much higher level of anxiety feature than gain. 
On average, commitment has the highest level of the anger and sad features, while authority has the lowest level of the sad feature (Figs.~\ref{app_fig_feature_vs_weapon_anger_liwc} and~\ref{app_fig_feature_vs_weapon_sad_liwc}).
Social proof has the lowest level of reward and risk (Figs.~\ref{app_fig_feature_vs_weapon_reward_liwc} and \ref{app_fig_feature_vs_weapon_risk_liwc}). %, and~\ref{app_fig_feature_vs_weapon_time_liwc}).
Figure~\ref{app_fig_feature_vs_weapon_risk_liwc} shows that loss, followed by authority, have a high level of risk feature. 
% Finally, while  authority and loss principles use money features most frequently, the principle of commitment barely mentions money-related words. %~\ref{app_fig_feature_vs_weapon_money_liwc}.

\begin{figure*}[htp]
    \centering
    \caption{\needsupdate LIWC features vs. principles of influence. For each category, the solid circle is the mean and the bar represents 95\% confidence interval.}
    \begin{subfigure}[b]{0.4\textwidth}
            \centering
            \includegraphics[width=\columnwidth]{fig/feature_plot/feature_vs_weapon/s00_feature_vs_weapon_anx_liwc}%
            \caption{Feature: \textit{anxiety}.}
        	\label{app_fig_feature_vs_weapon_anx_liwc}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.4\textwidth}
            \centering
            \includegraphics[width=\columnwidth]{fig/feature_plot/feature_vs_weapon/s01_feature_vs_weapon_anger_liwc}%
        	\caption{Feature: \textit{anger}.} %For each category, the solid circle is the mean and the bar represents 95\% confidence interval.}
        	\label{app_fig_feature_vs_weapon_anger_liwc}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.4\textwidth}
            \centering
            \includegraphics[width=\columnwidth]{fig/feature_plot/feature_vs_weapon/s02_feature_vs_weapon_sad_liwc}%
        	\caption{Feature: \textit{sad}.} %For each category, the solid circle is the mean and the bar represents 95\% confidence interval.}
        	\label{app_fig_feature_vs_weapon_sad_liwc}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.4\textwidth}
            \centering
            \includegraphics[width=\columnwidth]{fig/feature_plot/feature_vs_weapon/s03_feature_vs_weapon_reward_liwc}%
        	\caption{Feature: \textit{reward}.}% For each category, the solid circle is the mean and the bar represents 95\% confidence interval.}
        	\label{app_fig_feature_vs_weapon_reward_liwc}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.4\textwidth}
            \centering
            \includegraphics[width=\columnwidth]{fig/feature_plot/feature_vs_weapon/s04_feature_vs_weapon_risk_liwc}%
        	\caption{Feature: \textit{risk}.} % For each category, the solid circle is the mean and the bar represents 95\% confidence interval.}
        	\label{app_fig_feature_vs_weapon_risk_liwc}
    \end{subfigure}
    % \hfill
        % \includegraphics[width=0.9\columnwidth]{fig/feature_plot/feature_vs_weapon/s00_feature_vs_weapon_anx_liwc}\hfill%
        % \includegraphics[width=0.9\columnwidth]{fig/feature_plot/feature_vs_weapon/s01_feature_vs_weapon_anger_liwc}\hfill%
        % \includegraphics[width=0.9\columnwidth]{fig/feature_plot/feature_vs_weapon/s02_feature_vs_weapon_sad_liwc}\hfill%
        % \includegraphics[width=0.9\columnwidth]{fig/feature_plot/feature_vs_weapon/s03_feature_vs_weapon_reward_liwc}\hfill%
        % \includegraphics[width=0.9\columnwidth]{fig/feature_plot/feature_vs_weapon/s04_feature_vs_weapon_risk_liwc}\hfill%
\end{figure*}



% \begin{figure}[h!]
% 	\centering
% 	\includegraphics[width=\columnwidth]{fig/feature_plot/feature_vs_weapon/s00_feature_vs_weapon_anx_liwc}
% 	\caption{LIWC feature  ``\textbf{anxiety}'' vs. principles of influence. For each category, the solid circle is the mean and the bar represents 95\% confidence interval.}
% 	\label{app_fig_feature_vs_weapon_anx_liwc}
% \end{figure}


% \begin{figure}[h!]
% 	\centering
% 	\includegraphics[width=\columnwidth]{fig/feature_plot/feature_vs_weapon/s01_feature_vs_weapon_anger_liwc}
% 	\caption{LIWC feature ``\textbf{anger}'' vs. principle of influence.} %For each category, the solid circle is the mean and the bar represents 95\% confidence interval.}
% 	\label{app_fig_feature_vs_weapon_anger_liwc}
% \end{figure}


% \begin{figure}[h!]
% 	\centering
% 	\includegraphics[width=\columnwidth]{fig/feature_plot/feature_vs_weapon/s02_feature_vs_weapon_sad_liwc}
% 	\caption{LIWC feature ``\textbf{sad}'' vs. principle of influence.} %For each category, the solid circle is the mean and the bar represents 95\% confidence interval.}
% 	\label{app_fig_feature_vs_weapon_sad_liwc}
% \end{figure}

% \begin{figure}[h]
% 	\centering
% 	\includegraphics[width=\columnwidth]{fig/feature_plot/feature_vs_weapon/s03_feature_vs_weapon_reward_liwc}
% 	\caption{LIWC feature ``\textbf{reward}'' vs. influence principles.}% For each category, the solid circle is the mean and the bar represents 95\% confidence interval.}
% 	\label{app_fig_feature_vs_weapon_reward_liwc}
% \end{figure}

% \begin{figure}[h!]
% 	\centering
% 	\includegraphics[width=\columnwidth]{fig/feature_plot/feature_vs_weapon/s04_feature_vs_weapon_risk_liwc}
% 	\caption{LIWC feature ``\textbf{risk}'' vs. principles of influence.} % For each category, the solid circle is the mean and the bar represents 95\% confidence interval.}
% 	\label{app_fig_feature_vs_weapon_risk_liwc}
% \end{figure}


%--------------------------

% \begin{figure}[h!]
% 	\centering
% 	\includegraphics[width=\columnwidth]{fig/feature_plot/feature_vs_weapon/s05_feature_vs_weapon_time_liwc}
% 	\caption{LIWC feature ``\textbf{time}'' vs. principles of influence.}% For each category, the solid circle is the mean and the bar represents 95\% confidence interval.}
% 	\label{app_fig_feature_vs_weapon_time_liwc}
% \end{figure}

% \begin{figure}[h!]
% 	\centering
% 	\includegraphics[width=\columnwidth]{fig/feature_plot/feature_vs_weapon/s06_feature_vs_weapon_money_liwc}
% 	\caption{LIWC feature \textbf{``money''} vs. influence principles. For each category, the solid circle is the mean and the bar represents 95\% confidence interval.}
% 	\label{app_fig_feature_vs_weapon_money_liwc}
% \end{figure}

\subsection{Emotional Salience}
\needsupdate
We also analyzed whether emotional salience has indicative powers to predict the principles of influence. Liking has the highest level of positive emotion and the lowest level of negative emotion 
%, thus scoring lowest on  neutral emotion 
%(Figures~\ref{app_fig_feature_vs_weapon_pos_sia} and 
(Fig.~\ref{app_fig_feature_vs_weapon_neg_sia}). %and~\ref{app_fig_feature_vs_weapon_neu_sia}).
Conversely, commitment 
%scores highest on neutral emotion and 
shows the lowest level of positive emotion and moderate negative emotion.
Loss shows the highest negative emotion.% (Fig.~\ref{app_fig_feature_vs_weapon_neg_sia}).



\begin{figure*}[htp]
    \centering
    \caption{\needsupdate Emotional salience vs. principles of influence. The solid circle is the mean and the bar represents 95\% confidence interval.}
    \begin{subfigure}[b]{0.4\textwidth}
            \centering
            \includegraphics[width=\columnwidth]{fig/feature_plot/feature_vs_weapon/s07_feature_vs_weapon_pos_sia}
            \caption{\textit{Positive} emotional feature.}% For each category, the solid circle is the mean and the bar represents 95\% confidence interval.}
            \label{app_fig_feature_vs_weapon_pos_sia}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.4\textwidth}
            \centering
        	\includegraphics[width=\columnwidth]{fig/feature_plot/feature_vs_weapon/s08_feature_vs_weapon_neg_sia}
        	\caption{\textit{Negative} emotional feature.}% For each category, the solid circle is the mean and the bar represents 95\% confidence interval.}
        	\label{app_fig_feature_vs_weapon_neg_sia}
    \end{subfigure}
\end{figure*}






% \begin{figure}[h!]
% 	\centering
% 	\includegraphics[width=\columnwidth]{fig/feature_plot/feature_vs_weapon/s07_feature_vs_weapon_pos_sia}
% 	\caption{``\textbf{Positive}'' emotional feature  vs. principles of influence.}% For each category, the solid circle is the mean and the bar represents 95\% confidence interval.}
% 	\label{app_fig_feature_vs_weapon_pos_sia}
% \end{figure}

% \begin{figure}[h!]
% 	\centering
% 	\includegraphics[width=\columnwidth]{fig/feature_plot/feature_vs_weapon/s08_feature_vs_weapon_neg_sia}
% 	\caption{``\textbf{Negative}'' emotional feature  vs. principles of influence.}% For each category, the solid circle is the mean and the bar represents 95\% confidence interval.}
% 	\label{app_fig_feature_vs_weapon_neg_sia}
% \end{figure}

%\begin{figure}[h!]
%	\centering
%	\includegraphics[width=\columnwidth]{fig/feature_plot/feature_vs_weapon/s09_feature_vs_weapon_neu_sia}
%	\caption{\textbf{``Neutral''} emotional feature  vs. principles of influence. For each category, the solid circle is the mean and the bar represents 95\% confidence interval.}
%	\label{app_fig_feature_vs_weapon_neu_sia}
%\end{figure}

%\texbf{Interplay LIWC and Emotion Features.} We also compared LIWC and emotional features against emails with different levels of complexity (from Fig.~\ref{app_fig_single_vs_multiple_reward_liwc} to Fig.~\ref{app_fig_single_vs_multiple_neg_sia} in Appendix \ref{sec_appendix}).These figures show that, on average,  simple emails applying only  principle of influence usually show low levels of LIWC features and emotional salience, while complex emails applying more than one principle of influence have high level features.
%This is due to the average manipulation. 
%For the emails with single influence principle, the chosen features concentrate on a small proportion.
%Averaging over all emails with single influence, the mean will be low and the variance will be large.

\subsection{Lumen's Multi-label Prediction}
\needsupdate
This section describes our results in evaluating Lumen's multi-label prediction using the dataset.

\textbf{Pre-processing the dataset.} As described in Section \ref{sec:design-impl}, Lumen generates three types of features at its first hierarchical level (emotional salience, LIWC categories, and topic structure), which serve as input  for the learning-based prediction algorithm (Random Forest, for this analysis) at Lumen's second hierarchical level (Figure \ref{fig:lumen}). These features rely on the unstructured text  of the emails. 
However, different features need distinct preprocessing procedures. In our work, we used the Natural Language Toolkit (NLTK) \cite{nlt} to pre-process the dataset. For all three types of features, we first removed all the punctuation, special characters, digital numbers, and words with only one or two characters. Next, we tokenized each  email into a list of lowercase words.

For topic modeling features, we removed stopwords  (which provide little semantic information) and applied stemming (replacing a word's inflected form with its stem form) to further clean up word tokens.
%Stopwords of a language are the most commonly used but uninformative word~\cite{Gerlach2019infomration}, such as ``for'', ``the'' and ``but'', which appear almost every sentence of English document but provide very limited semantic information.
%Stopword removal generally leads to better performance of topic modeling algorithms~\cite{shi2019evaluation}.
%As a result, to infer more meaningful topic structure, stopword are removed for topic modeling algorithm.
%Stemming refers to the procedure of replacing the inflected forms of a word with the word's stem form or base form.
%For instance, ``learned'', ''learning'' and ``learns'' all come from the same word ``learn'', stemming is to reduce all three inflected forms to the base form ``learn'' in the text data.
%Without stemming, different inflected forms of the same word are different unique word in the vocabulary, which dilutes the information concentration in each document and limits the ability of topic modeling algorithms to infer meaningful topic structure.
%After stopword removal, 
For LIWC features, we matched each word in each  email with the pre-determined word list in each LIWC category. We also performed stemming  for LIWC features. We did not need to perform pre-processing for emotional salience because we applied NLTK ~\cite{Hutto2014}, which has its own tokenization and pre-processing procedures.

We also filtered out phishing emails with less than ten words since topic modeling results for extremely short documents are not reliable~\cite{shi2019evaluation}.
We were then left with 1,763 cleaned phishing emails, with 202,500 tokens across the corpus, and 12,773 unique words in the vocabulary.
%Without stopword removal and stemming for the  1,763 phishing documents, we will have 262,508 tokens in the corpus and 16,002 unique words in the vocabulary.
%We train and test Lumen based on the 1,763 documents.


%we are using off-the-shelf toolkit from NLTK based on the work of Hutto and Gilbert~\cite{Hutto2014}, which has its own tokenizatin and pre-processing procedure.

\textbf{Training and Testing.} Next, we split the 1,763 phishing emails into a training  and a testing set.
In learning models, hyper-parameters are of crucial importance because they control the structure or learning processing of the algorithms.
%Consequently, the values of hyper-parameters will have great impact on the performance of Lumen framework. 
Lumen applies two learning algorithms: an unsupervised topic modeling algorithm (Latent Dirichlet Allocation, LDA) on the first hierarchical level and Random Forest (RF)  on the second level, each one introducing their own types of hyper-parameters.
%Thus, there are two types of hyper-parameters for topic modeling and random forest.
Examples of hyper-parameters for LDA include the number of topics and the concentration parameters for Dirichlet distributions. For RF, examples of hyper-parameters are the number of trees and the maximum depth of a tree.
We also used the grid search approach  to find a better combination of hyper-parameters.
Note that due to time and computational power constraints, it is impossible to search all hyper-parameters and all their potential values. 
In this work, we only performed the grid search for number of topics (LDA) and the number of trees (RF).
The results show that the optimal number of topics is 10 and the optimal number of trees in RF is 200. 
Note that the optimal result is limited by the grid search space, which only contains a finite size of parameter combinations.

If we only trained and tested Lumen on one single pair of training and testing sets, there would be high risk of overfitting, i.e., the trained learning algorithm would perform exceptional well on a specific testing set and would have poor ability to generalize to other testing sets.
%In machine learning, overfitting means the trained learning algorithm performs exceptional well on a specific testing set and has a poor ability to generalize to other testing sets.
To lower the risk of overfitting, we used 5-fold cross-validation
%In 5-fold cross-validation, we randomly divide the entire phishing dataset into five (almost) equal-size subsets, and create five pairs of training and testing sets, with each subset serving as a testing dataset once and the other four serving as a training dataset.
and the final performance of the learning algorithm is the average performance over the five training and testing pairs. 

\begin{table}[h]
	\caption{\needsupdate Detection of influence results for different learning algorithms.}
	\centering
	\begin{tabular}{c|c|c}
		\hline
		Learning algorithm        &       $F1$-macro      &   $F1$-micro       \\ \hline \hline
		{\bf Lumen}                     &       {\bf 57.92}\%         &   {\bf 79.30}\%               \\ \hline
		Labeled-LDA               &       42.20\%         &   63.73\%              \\ \hline
		LSTM                  &       63.90\%         &   78.39\%              \\ \hline
		Na\"{\i}ve         &       33.96\%         &   38.27\%              \\ \hline
	\end{tabular}
	\label{table_learning_result}
\end{table}

We compared Lumen's  performance in predicting the principle(s) of persuasion and framing applied to a given email with three other document classification algorithms. 
The first  is Labeled-LDA, a semi-supervised variation of the original LDA algorithm~\cite{Ramage2009, VanderHeijden2019}.
When training Labeled-LDA, both the raw phishing email text and the human generated labels for persuasion and framing were input into the model.
%Then the trained Labeled-LDA model are used to predict the existence of principles of influence.
Compared to Lumen, Labeled-LDA only uses the word frequency information from the raw text data and has a very rigid assumption of the relation between the   word frequency information and the human generated labels, which limits its flexibility and prediction ability.
The second learning algorithm used in the comparison with Lumen was the Long Short-Term Memory (LSTM), which is a special form of recurrent neural network~\cite{cummins1999}.
When applying LSTM to text data, it simulates the learning process of a human.
LSTM takes the input data recurrently, regulates the flow of information, and determines what to past on to the next processing step and what to forget.
Since neural networks mainly deal with vector operations, we used word embedding matrix to transfer each word into vector space~\cite{NAILI2017340}.
The main shortcoming of neural network is that it works as a blackbox,  making it hard to understand the underlying mechanism.
The last algorithm used in the comparative evaluation was  a na\"{\i}ve algorithm, which serves as a base line. 
For the na\"{\i}ve approach, we randomly generated each label for each phishing email according to a Bernoulli distribution with equal probabilities for two outcomes.

As shown in Table~\ref{table_learning_result}, we used $F1$-score (both macro and micro) to quantify the performance the algorithms.
The three learning algorithms performed much better than the naive algorithm, which shows that ML is promising for retrieval of influence cues in emails.
%useful information from the text data of phishing emails and build connections between the text data and the human generated labels.
$F1$-micro calculates the global average, which obtains the precision and recall on the global scale then calculate the $F1$ score, while $F1$-macro calculates $F1$ score for each category then average them to get $F1$ score.
Lumen  presented the  best performance in terms of $F1$-micro score,  followed by LSTM.
LSTM performed better for the $F1$-macro, but Lumen presented better interpretability (discussed below).
Both Lumen and LSTM presented better performance than Labeled-LDA in both $F1$ scores.



\textbf{Interpretability of Lumen.} To show Lumen's ability to provide better understanding to practitioners, we trained it again with the dataset and the optimal hyper-parameter values from grid search.
After  training, Lumen provided both the relative importance of each input feature and the topic structure of the dataset without additional computational costs, which LSTM cannot provide because it operates as a black-box.

As shown in Table~\ref{table_important_feature}, the top-four important features in Lumen's prediction decision-making process are given.
Among these features, one is from LIWC features, two are from topic features and one is from emotional salience, which shows the validity for the choice of these three major types of input features.
The most importance features are "Money" (from LIWC, indicating possible reward) and is Topic-5,
%``Money'' feature from LIWC, which is followed by a topic 
a feature related to online accounts.
%Interestingly,  topic modeling  also selected a topic (Topic-7), which mainly contains  formatting words. This is likely because  our automatic web scraping software could not entirely parse some HTML elements in the emails.Topic07 also shows that Lumen can  help practitioners to explore the dataset, a capability not  available in black-box models, such as LSTM.
The ``Risk'' feature from LIWC and the positive sentiment feature shared comparable level of importance for Lumen.
In sum, Lumen's interpretability can allow a   better understand of both the  dataset and the decision-making process  Lumen undergoes, consequently  providing invaluable insights for  feature selection.


\begin{table*}[]
	\centering
	\caption{\needsupdate Important features for Lumen's prediction.}
	\begin{tabular}{p{4cm}|p{3cm}|p{7cm}}
		\hline
		Input feature name	&  Feature importance	&	Keywords	\\ \hline
		Money-liwc	&	0.095	& cheaper, bank, coupon, refund, credit		\\ \hline
		Topic-5	&	0.088	&	account, paypal, click, secure, update	\\ \hline
		%	Topic-7	&	0.072	&	import, class, width, font, height	\\ \hline
		Risk-liwc	&	0.070	&	danger, loss, defend, caution, avoid	\\ \hline
		Positive sentiment 	&	0.070	&	None	\\ \hline
	\end{tabular}
	\label{table_important_feature}
\end{table*}












% ----------------------------------------
% ----------------------------------------
% ARCHIVED TEXT FROM ORIGINAL SUBMISSION
% ----------------------------------------
% ----------------------------------------
% We then developed a coding manual that  allowed us to map principles of persuasion  and framing to the email text. An excerpt of the  coding manual is given in  Appendix~A Table~2\ref{app_table_code_manual}. 
% For example, an email was to be labeled as applying gain if it lured the user into a perception that acting on the email would potentially lead to some gain or reward, for example, an online discount. %An email was to be labeled as applying loss if the email text was attempting to convince the user that not acting on the email could potentially cause a loss, e.g., account suspension.

% Two lead coders trained a team of six coders over a period of three weeks using the coding manual. The coders’ training comprehension was tested using 20 emails that were chosen by the trainers as representative of the principles of persuasion and framing. Coders were considered ready once labeling agreement was achieved on these representative emails. Because multiple principles of persuasion can be present within an individual email, Cohen's kappa was not computed to measure reliability. Instead, for each given email, two randomly assigned coders needed to reach an agreement on the labeling of a given email.  

% The emails were added to the database, reshuffled, and given a ‘coding order’ index value.  When a coder opened  the coding application with their id, the application found the next uncoded and unassigned email in the coder order. A web app was created that allowed the coders to read and label each email. The app also allowed coders to address any inconsistencies in their labeling. 
% We provide in the Appendix~A %\ref{sec_appendix} 
% examples of the web app in Figure~1 %\ref{app_fig_Screenshot_of_coding_an_email} 
% and the distribution of emails coded (randomly selected) in Table~1. %\ref{app_table_email_found_coded}. 
% Each week, coders referred to the “Reports” page of the coding app and checked for mismatches in labeling from the previous week’s labeling.  When mismatches existed, the coders met and worked through the reasoning behind their label based on the coding manual (Appendix~A, Table~2). % \ref{app_table_code_manual}.

% The coders labeled a total of  1,932  phishing emails over a period of approximately six months. After the coding process  concluded, there were 68 emails for which the coders did not find any of principles of influence (persuasion or framing) applied (3.5\% of the dataset). We manually inspected these 68 emails and found that they were composed of short statements or orders, which are too simple to include any sophisticated influence principle (e.g.,  ``\emph{cell phone voice message from office caller please click listen for free}''). After removal of these simple phishing emails our dataset was left with 1,864 email for which the coders found at least on principle of influence applied. 



==> sections/tmp5-results.tex <==
\section{Results}
\label{sec:eval}

This section details Lumen’s evaluation. We provide a quantitative analysis of the dataset, and the results of Lumen classification in comparison to other ML algorithms.


% ******************************
% ******************************
% ******************************
\subsection{Quantitative Analysis of the Dataset}
% ******************************
% ******************************
% ******************************
\changed{We first begin by quantifying the our curated dataset of nearly 3K deceptive, hyperpartisan, or mainstream texts, hand-labeled by a group of coders. When considering all influence cues, most texts used between three and six cues per texts; only 3\% of all texts leveraged a single influence cue, and 2\% used zero cues ($n=58$).}

\changed{When considering the most common pairs and triplets between all influence cues, slant (i.e., \emph{subjectivity} or \emph{objectivity}) and principles of persuasion (PoP) dominated the top 10 most common pairings and triplets. As such, the most common pairs were \emph{(authority, objectivity)} and \emph{(authority, subjectivity)}, occurring for 48\% and 45\% of all texts, respectively; this is due to both PoP and slant were the most commonly occurring influence cues in the dataset (as explained in the following subsections). The most common (PoP, PoP) pairing was between \emph{authority} and \emph{commitment}, co-occurring in 41\% of all texts. \emph{Emphasis} appeared once in the top 10 pairs and twice in the top triplets: \emph{(emphasis, subjectivity)} occurring for 29\% of texts, and \emph{(emphasis, authority, subjectivity)} and \emph{(emphasis, commitment, subjectivity)} for 20\% and 19\% of texts, respectively. \emph{Blame/guilt} appeared only once in  the top triplets as \emph{(authority, blame/guilt, objectivity)}, representing 19\% of all texts. \emph{Gain} framing appeared only as the 33rd most common pair \emph{(gain, subjectivity)} and 18th most common triplet \emph{(call to action, scarcity, gain)}, further emphasizing its scarcity in our dataset.}



% ******************************
% ******************************
% ******************************
\changed{\subsubsection{Principles of Persuasion}}
% ******************************
% ******************************
% ******************************
\changed{We found that most texts in the dataset contained one to four principles of persuasion, with only 4\% containing zero and 3\% containing six or more PoP labels (Fig.~\ref{fig:total_PoP_labels}); 29\% of texts apply two PoP and 23\% leverage three PoP. Further, Fig.~\ref{fig:pop_breakdown} shows that \emph{authority} and \emph{commitment} were the most prevalent principles appearing, respectively, in 71\% and 52\% of the texts; meanwhile, \emph{reciprocation} and \emph{indignation} were the least common PoP (5\% and 9\%, respectively).}


\begin{figure}[h]
	\centering
	\includegraphics[width=.75\columnwidth,trim={0 0 0 0.2cm}, clip]{fig/total_pop_per_text.png}
	\caption{\changed{Total number of principle of persuasion labels per each individual text. We see that 88\% of the texts contain one to four PoP labels.} \commentario{Upload high res version.}}
	\label{fig:total_PoP_labels}
\end{figure}

\changed{Almost all types of texts contained every PoP to varying degrees (Fig.~\ref{fig:pop_breakdown_per_type}); the only exception is \emph{reciprocation} (the least-used PoP overall) which was not at all present in fake news texts (in the Deceptive Texts Group) and barely present ($n=3$, 0.6\%) in right-leaning hyperpartisan news. \emph{Authority} was the most-used PoP for all types of texts, except phishing emails (most: \emph{call to action}) and IRA ads (most: \emph{commitment}), both of which are in the Deceptive Texts Group.}




\begin{figure*}[h]
  \centering
  \subfloat[\changed{The total for each principle of persuasion label, broken down based on type of text.}]{\includegraphics[width=0.5\textwidth]{fig/pop_breakdown_total_texts.png}\label{fig:pop_breakdown}}
  \hfill
  \subfloat[\changed{The total for each text type, broken down based on principles of persuasion.}]{\includegraphics[width=0.5\textwidth]{fig/pop_breakdown_total_texts_per_type.png}\label{fig:pop_breakdown_per_type}}
  \caption{\changed{Breakdown of principle of persuasion and text type.} \commentario{Upload high res version.}}
\end{figure*}





% \noindent
\changed{{\bf Deceptive Texts.} Fake news was notably reliant on \emph{authority} (92\% of all fake news contained the \emph{authority} label) compared to phishing emails (45\%) and the IRA ads (32\%); however, fake news used \emph{liking, reciprocation}, and \emph{scarcity} (5\%, 0\%, 3\%, respectively) much less often than phishing emails (27\%, 8\%, 65\%) or IRA ads (41\%, 10\%, 24\%). Interestingly, \emph{admonition} was most used by fake news (35\%), though overall, \emph{admonition} was only present in 14\% of all texts. Phishing emails were noticeably more reliant on \emph{call to action} (80\%) and \emph{scarcity} (65\%) compared to fake news (33\%, 3\%) and IRA ads (40\%, 24\%), yet barely used \emph{indignation} (0.4\%) compared to the same (13\% for fake news and 17\% for IRA ads). The IRA ads relied on \emph{indignation, liking, reciprocation}, and \emph{social proof} much more than the others; note again that \emph{reciprocation }was the least occurring PoP (5\% overall), but was most commonly occurring in IRA ads (10\%). }

\changed{{\bf Hyperpartisan News.} Right-learning texts had nearly twice as much \emph{call to action} and \emph{indignation} than left-leaning texts (61\% and 19\% vs. 31\% and 8\%, respectively). Meanwhile, left-learning hyperpartisan texts had noticeably more \emph{liking} (30\% vs. 13\%), \emph{reciprocation} (8\% vs. 0.6\%), and \emph{scarcity} (27\% vs. 13\%) than right-learning texts. 
}

\changed{{\bf Mainstream News.} \emph{Authority} (88\%) and \emph{commitment} (43\%) were the most frequently appearing PoP in center news, though this represents the third highest occurrence of \emph{authority} and lowest use of \emph{commitment} across all six text type groups.  Mainstream news also used very little \emph{indignation} (3\%) compared the the other text types except phishing emails (0.4\%), and also demonstrated the lowest use of \emph{social proof} (7\%).}


\changed{Lastly, Fig.~\ref{fig:pop_pairs} shows the most commonly occurring pairs of principles of persuasion. The \emph{authority} and \emph{commitment} principles co-occurred for 41\% of the texts, followed by \emph{authority} and \emph{call to action} for 28\% of texts. \emph{Call to action }and \emph{scarcity} was the fourth most common pair (19\%), and \emph{authority} and \emph{liking} were the seventh most common pair (14\%). 
}

\begin{figure}[h]
	\centering
	\includegraphics[width=1.0\columnwidth,trim={0 0 0 0.2cm}, clip]{fig/pop_pairs_balloonplot.png}
	\caption{\changed{The co-occurrances (i.e., frequency of pairings) of principle of persuasion labels.}\commentario{Upload High res version.}}
	\label{fig:pop_pairs}
\end{figure}



\takeaway{\changed{\emph{Authority} and \emph{commitment} were the most common principles of persuasion in the dataset, however, the use PoP varied within each text group. While \emph{authority} was the top PoP for the Mainstream and Hyperpartisan News Groups, the Deceptive Texts group showed variation: phishing emails had the largest occurrence of \emph{scarcity} and IRA ads had the largest occurrence of \emph{commitment}. Hyperpartisan news had nearly opposing PoP frequencies (e.g., high occurrence of \emph{reciprocation} for left-leaning but low occurrence for right-learning media). The most common PoP pairs involved either \emph{commitment}, \emph{call to action}, or \emph{authority}, i.e., the most frequently occurring PoP in the dataset. }}









% ******************************
% ******************************
% ******************************
\changed{\subsubsection{Framing}}
% ******************************
% ******************************
% ******************************
\changed{There were few \emph{gain} or \emph{loss} labels for the overall dataset (only 13\% and 7\%, respectively). Very few texts (18\%) were framed exclusively as either \emph{gain} or \emph{loss}, 81\% did not include any framing at all, and only 1\% of the texts used both \emph{gain} and \emph{loss} framing in the same message. We also found that \emph{gain} was much more prevalent than \emph{loss} across all types of texts, with the exception of fake news, which showed an equal amount (1.5\% for both \emph{gain} and \emph{loss}). Notably, phishing emails had significantly more \emph{gain} and \emph{loss} than any other text type (41\% and 29\%, respectively); mainstream center news and IRA ads showed some use of \emph{gain} framing (10\% and 13\%, respectively) compared to the remaining text types.}


\changed{Next, we investigated how persuasion and framing were used in texts by analyzing the pairs and triplets between the two influence cues. \emph{Gain} framing most frequently occurred with \emph{call to action} and \emph{commitment}, though these represent only 9\% of pairings. \emph{Gain, call to action} and \emph{scarcity} was the the most common triplet between PoP and framing, occurring for 7\% of all texts—this is notable as phishing emails had \emph{call to action} and \emph{scarcity} as its top PoP, and \emph{gain} framing was also most prevalent in phishing. Also of note is that \emph{loss} appeared in even fewer common pairs and triplets compared to \emph{gain} (e.g., \emph{loss} and \emph{call to action} appeared in just 5\% of texts).}

\takeaway{\changed{Framing was a relatively rare occurrence in the dataset, though framing was predominantly present in phishing emails, wherein \emph{gain} was invoked $1.5\times$ as often as \emph{loss}.}}




% ******************************
% ******************************
% ******************************
\subsubsection{Emotional Salience}
% ******************************
% ******************************
% ******************************
\changed{We used VADER’s compound sentiment score ($E$, wherein $E\geq0.05$, , $E\leq-0.05$, and $-0.05<  E < 0.05$ denote positive, negative, and neutral sentiment, respectively) and LIWC’s positive and negative emotion word count metrics to measure sentiment. Overall, our dataset was slightly positive in terms of average compound sentiment ($\mu=0.23$) and with an average of 4.0 positive emotion words and 1.7 negative emotion words per text.}

\changed{In terms of specific text types, fake news contained the only negative average compound sentiment ($-0.163$), and right-leaning hyperpartisan news had the only neutral average compound sentiment ($0.015$); all other text types had, on average, positive sentiment, with phishing emails as the most positive text type ($0.635$). Left-leaning hyperpartisan news had the highest average positive emotion word count ($5.649$) followed by phishing emails ($4.732$), whereas fake news had the highest average negative word count ($2.892$) followed by left hyperpartisan news ($2.796$).}

We also analyzed whether emotional salience has indicative powers to predict the \changed{influence cues (Fig.~\ref{fig:sentiment_influence_cues}). The majority of the influence cues and LIWC categories had an average positive sentiment, with \emph{liking} and \emph{gain} framing having the highest levels of positive emotion. \emph{Anxiety} and \emph{anger} (both LIWC categories) showed the only neutral sentiment, whereas \emph{admonition, blame/guilt}, and \emph{indignation} as the only negative sentiment (with the latter being the most negative out of all categories). Interestingly, items such as \emph{loss} framing and LIWC’s \emph{risk} both had positive sentiment.}


\begin{figure}[h]
	\centering
	\includegraphics[width=1.0\columnwidth,trim={0 0 0 0.2cm}, clip]{fig/sentiment_influence_cues.png}
	\caption{\changed{Average sentiment (measured by VADER’s compound score) for each influence cue and LIWC categories. The green and red horizontal lines indicate where positive and negative sentiment begin (at $y=0.05$ and $y=-0.05$, respectively).} \commentario{Upload high res version}}
	\label{fig:sentiment_influence_cues}
\end{figure}


\takeaway{\changed{The dataset invoked an overall positive sentiment, with phishing emails containing the most positive average sentiment and fake news with the most negative average sentiment. In terms of influence cues, we again saw a majority positive sentiment, especially in the cases of \emph{liking} and \emph{gain} framing; conversely, \emph{admonition, blame/guilt}, and \emph{indignation} contained the most negative sentiments.}}





% ******************************
% ******************************
% ******************************
\changed{\subsubsection{Slant}}
% ******************************
% ******************************
% ******************************
\changed{The \emph{objective} and \emph{subjective} labels were present in 52\% and 64\% of all texts in the dataset, respectively. This $>50$\% frequency for both categories was present in all text types except phishing emails and IRA ads, where \emph{subjectivity} was approximately $2.5\times$ more common than \emph{objectivity}. The most subjective text type were IRA ads (77\%) and the most objective texts were fake news (72\%); inversely, the least objective texts were phishing emails (27\%) and least subjective were mainstream center news (58\%). 
}

\changed{More notably, there was an overlap between the slants, wherein 29\% of all texts contained both \emph{subjective} and \emph{objective} labels. This could be a reflection of mixing factual (objective) statements with subjective interpretations of them. Nonetheless, \emph{objectivity} and \emph{subjectivity} were independent variables, $\chi^2 (4, N=2,998) = 72.0, p \approx 0$. The parings \emph{(objectivity, authority)} and \emph{(subjectivity, authority)} were the the top two most common pairs considering PoP and slant; these pairs occurred at nearly the same frequency within the dataset (48\% and 45\%, respectively). This pattern repeats itself for other (PoP, slant) pairings and triplets, insofar as \emph{(objectivity, subjectivity, authority)} is the third most commonly occurring triplet. When comparing just (PoP, slant) triplets, slant is present in $9/10$ top triplets, with \emph{(subjectivity, authority, commitment)} and \emph{(objectivity, authority, commitment)} as the two most common triplets (30\% and 27\%, respectively). 
}

\takeaway{\changed{The \emph{objectivity} and \emph{subjectivity} were independent labels that often co-occurred in the same texts, and appeared most frequently alongside \emph{commitment} and \emph{authority}.}}





% ******************************
% ******************************
% ******************************
\changed{\subsubsection{Attribution of Blame \& Guilt}}
% ******************************
% ******************************
% ******************************
\changed{Twenty-nine percent of all texts contained the \emph{blame/guilt} label. Interestingly, nearly the same proportions of fake news (45.4\%) and right-leaning hyperpartisan news (45.0\%) were labeled with \emph{blame/guilt}, followed by left-leaning hyperpartisan news (38\%). Phishing emails, IRA ads, and mainstream center media used \emph{blame/guilt} at the lowest frequencies (ranging from 15\% to 25\%). }

\changed{\emph{Blame/guilt} was somewhat seen in the top 10 pairs with PoP, only pairing with \emph{authority} (4th most common pairing with 26\% frequency) and \emph{commitment} (6th most common, 18\%). However, \emph{blame/guilt} appeared more frequently amongst the top 10 triplets with PoP, co-occurring with \emph{authority, commitment, call to action,} and \emph{social admonition}.}

\takeaway{\changed{\emph{Blame/guilt} did not appear frequently in our dataset, but appeared in higher proportions for fake and hyperpartisan news. It most commonly co-occurred with \emph{authority }or \emph{commitment}.}}







% ******************************
% ******************************
% ******************************
\changed{\subsubsection{Emphasis}}
% ******************************
% ******************************
% ******************************
\changed{\emph{Emphasis} was used in nearly 35\% of all texts in the dataset. Among them, all news sources (fake, hyperpartisan, and mainstream) appeared with the smallest use of \emph{emphasis} (range: 17\% to 26\%). This follows as news (regardless of veracity) likely is attempting to purport itself as legitimate. On the other hand, phishing emails and IRA ads were both shared on arguably more informal environments of communication (email and social media), and were thus often found to use emphasis (over 54\% for both categories). Additionally, similar to previous analyses for other influence cues, \emph{emphasis} largely co-occurred with \emph{authority, commitment,} and \emph{call to action}.}

\takeaway{\changed{The use of emphasis was much more common in informal text typed (phishing emails and IRA social media ads), and less common in news-like sources (fake, hyperpartisan, or mainstream).}}








% ******************************
% ******************************
% ******************************
\subsubsection{LIWC Features of Influence}
% ******************************
% ******************************
% ******************************
We also explored whether LIWC features have indicative powers to predict the \changed{influence cues. Table~\ref{tab:LIWC_influence} shows that \emph{indignation} and \emph{admonition} had the highest average \emph{anxiety} feature, while \emph{liking} and \emph{gain} framing had the lowest. \emph{Indignation} also scored three times above the overall average for the \emph{anger} feature, as well as for \emph{sadness} (alongside \emph{blame/guilt}), whereas \emph{gain} had the lowest average for both \emph{anger} and \emph{sadness}. The \emph{reward} feature was seen most in \emph{liking} and in \emph{gain}, while \emph{risk} was slightly more common in \emph{loss} framing. The \emph{time} category had the highest overall average and was most common in \emph{blame/guilt}, while \emph{money} had the second largest overall average and was most common in \emph{loss}.}

\input{tables/tab:LIWC_influence}

\changed{We also saw that that left-leaning hyperpartisan news had the highest average \emph{anxiety}, \emph{sadness}, \emph{reward}, and \emph{time} counts compared to all text types, whereas right-learning hyperpartisan news averaged slightly higher than left-leaning media only in the \emph{risk} feature. Note, however, that LIWC is calculated based on word counts and is therefore possibly biased towards longer length texts; it should thus be noted that while hyperpartisan left media had the highest averages for four of the seven LIWC features, hyperpartisan media also had the second largest average text length compared to other text types.}


\changed{For the Deceptive Texts Group, phishing emails had the largest \emph{risk} and \emph{money} averages over all text types, while averaging lowest in \emph{anxiety}, \emph{anger}, and \emph{sadness}. Fake news was highest overall in \emph{anger}, though it was slightly higher in \emph{anxiety}, \emph{sadness}, and \emph{time} compared to phishing emails and IRA ads. On the other hand, the IRA ads were lowest in \emph{reward}, \emph{risk}, \emph{time}, and \emph{money} compared to the its group.}

\changed{Lastly, mainstream center media had no LIWC categories in either high or low extremities—most of its average LIWC values were close to the overall averages for the entire dataset.}


\takeaway{\changed{The seven LIWC influence features varied depending on both influence cues and on types of text. Left hyperpartisan news had the highest averages for four features (\emph{anxiety}, \emph{sadness}, \emph{reward}, and \emph{time}). In terms of influence cues, \emph{indignation} had the highest averages for three features (\emph{anxiety}, \emph{anger}, and \emph{sadness}), and \emph{loss} framing (\emph{risk} and \emph{money}) and \emph{blame/guilt} (\emph{sadness} and \emph{time}) for two features each.}}









% ******************************
% ******************************
% ******************************
\subsection{Lumen's Multi-Label Prediction}
% ******************************
% ******************************
% ******************************
\commentario{@Hanyu: Please update this sub-section with results.}

This section describes our results in evaluating Lumen's multi-label prediction using the dataset.








% ******************************
% ******************************
% ******************************
\changed{\subsubsection{ML Algorithms}}
% ******************************
% ******************************
% ******************************

\changed{We compared Lumen’s performance against three other ML algorithms: Labeled-LDA, LSTM, and a naïve algorithm.} The former two learning algorithms and Lumen performed much better than the naive algorithm, which shows that ML is promising for retrieval of influence cues in texts. 
Lumen presented the best performance in terms of $F1$-micro score (\commentario{value here}), followed by LSTM (\commentario{value here}). This indicates that \XXX. 

\input{tables/tab:learning_results}

On the other hand, LSTM outperformed Lumen in terms of $F1$-macro \changed{(\commentario{value here} and \commentario{value here}, respectively), thus potentially indicating that \XXX. Nonetheless,} Lumen presented better interpretability (discussed below).

Finally, both Lumen and LSTM presented better performance than Labeled-LDA in both $F1$ scores, \changed{further emphasizing that \XXX.}

\commentario{@Hanyu: also talk about the confusion matrix and accuracy + any other evaluation metrics.}

\changed{These results are summarized in Table~\ref{tab:learning_result}.}









% ******************************
% ******************************
% ******************************
\subsubsection{Interpretability of Lumen} 
% ******************************
% ******************************
% ******************************
\commentario{Items in red are old results.}

To show Lumen's ability to provide better understanding to practitioners, we trained it with our dataset and the optimal hyper-parameter values from grid search. After  training, Lumen provided both the relative importance of each input feature and the topic structure of the dataset without additional computational costs, which LSTM cannot provide because it operates as a black-box.

Table~\ref{tab:important_feature} shows the top-four important features in Lumen's prediction decision-making process. Among these features, \commentario{one is from {LIWC features}, two are from topic features and one is from emotional salience}, which shows the validity for the choice of these three major types of input features. The most important features are \commentario{\textit{money} (from LIWC, indicating possible reward) and is \textit{Topic-5} (from topic modeling, related to online accounts). The \textit{risk} feature from LIWC and the positive sentiment feature shared comparable level of importance for Lumen.}

==> tables/tab_input_feature.tex <==
\begin{table}[h]
\centering
\caption{Input features for each text, $d$.}
\label{tab:input_feature}
\begin{tabular}{@{}ccc@{}}
\toprule
\textbf{Features} & \textbf{Symbols}                            & \textbf{Number of features} \\ \midrule
Topic             & $P(t|d), i=1,...,K$                         & $K$                         \\
LIWC              & $X^{LIWC}_{i,d}, \forall i \in \mathcal{S}$ & 7                           \\
Emotion           & $E^{pos}_d$, $E^{neg}_d$                    & 2                           \\ \bottomrule
\end{tabular}
\end{table}

==> tables/tab_liwc_cats.tex <==
\begin{table}[h]
\centering
\caption{LIWC categories and keywords.}
\label{tab:liwc_cats}
\begin{tabular}{ccc}
\toprule
\textbf{LIWC Category} & \textbf{Keywords} & \textbf{Total Words} \\ \midrule
\textit{Anxiety}       & afraid, anxious   & 92                   \\
\textit{Anger}         & abuse, aggress    & 176                  \\
\textit{Sadness}       & abandon, alone    & 98                   \\
\textit{Time}          & after, afternoon  & 251                  \\
\textit{Reward}        & access, achieve   & 75                   \\
\textit{Risk}          & alarm, abstain    & 81                   \\
\textit{Money}         & account, auction  & 167                  \\ \bottomrule
\end{tabular}
\end{table}
